Unified properties of supermassive black hole winds in radio-quiet and radio-loud AGN

Powerful supermassive black hole (SMBH) winds in the form of ultra-fast outflows (UFOs) are detected in the X-ray spectra of several active galactic nuclei (AGN) seemingly independently of their radio classification between radio quiet (RQ) and radio loud (RL). In this work we explore the physical parameters of SMBH winds through a uniform analysis of a sample of X-ray bright RQ and RL AGN. We explored several correlations between different wind parameters and with respect to the AGN bolometric and Eddington luminosities. Our analysis shows that SMBH winds are not only a common trait of both AGN classes but also that they are most likely produced by the same physical mechanism. Consequently, we find that SMBH winds do not follow the radio-loudness dichotomy seen in jets. On average, a comparable amount of material accreted by the SMBH is ejected through such winds. The average wind power corresponds to about 3 per cent of the Eddington luminosity, confirming that they can drive AGN feedback. Moreover, the most energetic outflows are found in the most luminous sources. We find a possible positive correlation of the wind energetics, renormalized to the Eddington limit, with respect to $\lambda_{Edd}$, consistent with the correlation found with bolometric luminosity. We also observe a possible positive correlation between the energetics of the outflow and the X-ray radio-loudness parameter. In general, these results suggest an underlying relation between the acceleration mechanisms of accretion disc winds and jets.

==> name.tex <==
1 & 3.35	$\pm$	1.27	&	-2.15	$\pm$	1.27	&	0.65	$\pm$	1.27	&	-0.77	$\pm$	1.27	&	0.61	$\pm$	1.27\\
2 & 3.95	$\pm$	1.71	&	-1.95	$\pm$	1.71	&	0.07	$\pm$	1.71	&	-0.41	$\pm$	1.71	&	-0.05	$\pm$	1.71\\
3 & 2.42	$\pm$	1.30	&	-0.70	$\pm$	1.30	&	0.16	$\pm$	1.30	&	-0.28	$\pm$	1.30	&	0.60	$\pm$	1.30\\
4 & 3.34	$\pm$	2.06	&	-0.87	$\pm$	2.06	&	0.47	$\pm$	2.06	&	-0.28	$\pm$	2.06	&	0.82	$\pm$	2.06\\
5 & 1.83	$\pm$	0.16	&	-2.17	$\pm$	0.16	&	0.41	$\pm$	0.16	&	-1.20	$\pm$	0.16	&	0.57	$\pm$	0.16\\
6 & 2.90	$\pm$	0.37	&	-2.32	$\pm$	0.37	&	1.04	$\pm$	0.37	&	-0.49	$\pm$	0.37	&	0.78	$\pm$	0.37\\
7 & 4.60	$\pm$	1.66	&	-1.12	$\pm$	1.66	&	2.43	$\pm$	1.66	&	1.12	$\pm$	1.66	&	1.96	$\pm$	1.66\\
8 & 3.64	$\pm$	1.13	&	-2.80	$\pm$	1.13	&	-0.18	$\pm$	1.13	&	-1.00	$\pm$	1.13	&	-0.43	$\pm$	1.13\\
9 & 4.00	$\pm$	2.27	&	-1.67	$\pm$	2.27	&	0.39	$\pm$	2.27	&	-0.65	$\pm$	2.27	&	0.53	$\pm$	2.27\\
10 & 1.96	$\pm$	0.65	&	-1.19	$\pm$	0.65	&	0.17	$\pm$	0.65	&	-0.58	$\pm$	0.65	&	0.51	$\pm$	0.65\\
11 & 3.95	$\pm$	1.46	&	-1.86	$\pm$	1.46	&	0.08	$\pm$	1.46	&	-0.07	$\pm$	1.46	&	-0.17	$\pm$	1.46\\
12 & 3.76	$\pm$	0.58	&	-3.24	$\pm$	0.58	&	0.64	$\pm$	0.58	&	-0.76	$\pm$	0.58	&	0.05	$\pm$	0.58\\
13 & 3.26	$\pm$	1.02	&	-2.68	$\pm$	1.02	&	0.24	$\pm$	1.02	&	-1.14	$\pm$	1.02	&	0.13	$\pm$	1.02\\
14 & 1.95	$\pm$	0.74	&	-1.26	$\pm$	0.74	&	0.58	$\pm$	0.74	&	-0.74	$\pm$	0.74	&	0.97	$\pm$	0.74\\
15 & 2.25	$\pm$	1.12	&	-1.02	$\pm$	1.12	&	0.62	$\pm$	1.12	&	-0.60	$\pm$	1.12	&	1.05	$\pm$	1.12\\
16 & 2.67	$\pm$	1.40	&	-1.02	$\pm$	1.40	&	0.33	$\pm$	1.40	&	-0.45	$\pm$	1.40	&	0.69	$\pm$	1.40\\
17 & 2.45	$\pm$	0.44	&	-2.85	$\pm$	0.44	&	-0.32	$\pm$	0.44	&	-1.54	$\pm$	0.44	&	-0.33	$\pm$	0.44\\
18 & 2.02	$\pm$	0.02	&	-2.40	$\pm$	0.02	&	0.57	$\pm$	0.02	&	-1.10	$\pm$	0.02	&	0.57	$\pm$	0.02\\
19 & 2.76	$\pm$	1.68	&	-1.60	$\pm$	1.68	&	-0.28	$\pm$	1.68	&	-1.22	$\pm$	1.68	&	0.17	$\pm$	1.68\\
20 & 2.66	$\pm$	0.59	&	-1.74	$\pm$	0.59	&	0.88	$\pm$	0.59	&	-0.37	$\pm$	0.59	&	0.84	$\pm$	0.59\\
21 & 3.62	$\pm$	1.10	&	-2.74	$\pm$	1.10	&	-0.85	$\pm$	1.10	&	-0.92	$\pm$	1.10	&	-1.11	$\pm$	1.10\\
22 & 2.90	$\pm$	0.70	&	-1.75	$\pm$	0.70	&	0.52	$\pm$	0.70	&	-0.24	$\pm$	0.70	&	0.42	$\pm$	0.70\\
23 & 2.34	$\pm$	0.77	&	-1.19	$\pm$	0.77	&	0.93	$\pm$	0.77	&	-0.31	$\pm$	0.77	&	1.14	$\pm$	0.77\\
24 & 3.25	$\pm$	1.61	&	-0.89	$\pm$	1.61	&	0.55	$\pm$	1.61	&	0.05	$\pm$	1.61	&	0.73	$\pm$	1.61\\
25 & 2.68	$\pm$	0.81	&	-2.10	$\pm$	0.81	&	0.47	$\pm$	0.81	&	-0.93	$\pm$	0.81	&	0.54	$\pm$	0.81\\
26 & 3.27	$\pm$	1.87	&	-1.46	$\pm$	1.87	&	-0.64	$\pm$	1.87	&	-0.75	$\pm$	1.87	&	-0.34	$\pm$	1.87\\
27 & 2.58	$\pm$	1.49	&	-0.27	$\pm$	1.49	&	2.04	$\pm$	1.49	&	0.12	$\pm$	1.49	&	2.49	$\pm$	1.49\\






